Why So Pessimistic? Estimating Uncertainties for Offline RL through Ensembles, and Why Their Independence Matters

Motivated by the success of ensembles for uncertainty estimation in supervised learning, we take a renewed look at how ensembles of $Q$-functions can be leveraged as the primary source of pessimism for offline reinforcement learning (RL). We begin by identifying a critical flaw in a popular algorithmic choice used by many ensemble-based RL algorithms, namely the use of shared pessimistic target values when computing each ensemble member's Bellman error. Through theoretical analyses and construction of examples in toy MDPs, we demonstrate that shared pessimistic targets can paradoxically lead to value estimates that are effectively optimistic. Given this result, we propose MSG, a practical offline RL algorithm that trains an ensemble of $Q$-functions with independently computed targets based on completely separate networks, and optimizes a policy with respect to the lower confidence bound of predicted action values. Our experiments on the popular D4RL and RL Unplugged offline RL benchmarks demonstrate that on challenging domains such as antmazes, MSG with deep ensembles surpasses highly well-tuned state-of-the-art methods by a wide margin. Additionally, through ablations on benchmarks domains, we verify the critical significance of using independently trained $Q$-functions, and study the role of ensemble size. Finally, as using separate networks per ensemble member can become computationally costly with larger neural network architectures, we investigate whether efficient ensemble approximations developed for supervised learning can be similarly effective, and demonstrate that they do not match the performance and robustness of MSG with separate networks, highlighting the need for new efforts into efficient uncertainty estimation directed at RL.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sass.tex <==
\section{Adding some SASS}
\label{app:sass}
\textbf{Please note that for all results reported in this work, outside of this section, we did not use the SASS objective.}

\begin{figure}[t]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/no_sass (3).pdf}
        \caption{
            No Sass
        }
        \label{fig:no_sass_appendix}
    \end{minipage}\hfill
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/with_sass.pdf}
        \caption{
            With Sass
        }
        \label{fig:with_sass}
    \end{minipage}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/no_sass_vs_with_sass.pdf}
    \caption{Caption}
    \label{fig:no_sass_vs_with_sass}
\end{figure}

In the derivations of Appendix \ref{app:proof}, a key term that appears in a number of equations is $(1 + \ldots + \gamma^{t} C^{t})$, where,
    \begin{align*}
        C &:= \tzero(\exprime, \ex) \cdot \tzero(\mathcal{X}, \mathcal{X})^{-1}\\
        \tzero(A, B) &:= \nabla_\theta Q_{\theta}(A)  \cdot \nabla_\theta Q_{\theta}(B)^T \vert_{t=0}
    \end{align*}
Throughout our derivations we assumed that the spectral norm of $C$ is less than $\frac{1}{\gamma}$, so that the geometric term above does not diverge through the iterations of fitted policy evaluation. Intuitively, we hypothesize that regularizing the $C$ matrix to ensure this condition would be beneficial for offline policy evaluation as well as offline RL. We have attempted a variety of approaches to effectively perform spectral norm regularization the $C$ matrix. Here, we outline the most promising approach we have found, which we will refer to as "State-Action-State Spectral norm regularization" (SASS).

\subsection{The SASS Regularizer}
In the infinite-width limit, these two matrices are obtained from the Neural Tangent Kernel \citep{jacot2018neural} which does not change throughout training. Hence, we focus our attention on how to perform this regularization in the practical setting, with finite-width networks and using mini-batches as opposed to full-batch training.

As opposed to the infinite-width setting, with finite networks, the outerproduct given by $\hat{\Theta}^{(t)}(A, B) := \nabla_\theta Q_{\theta}(A) \cdot \nabla_\theta Q_{\theta}(B)^T \vert_{\theta=\theta^{(t)}}$ changes after every training step $t$ as the parameters are updated. For this reason, we aimed to design a regularizing loss function to optimize w.r.t. $\theta^{(t)}$.

One naive approach we can consider is to regularize $\nabla_\theta Q_{\theta}(A) \cdot \nabla_\theta Q_{\theta}(B)^T$ to be close to identity matrices. Since the vectors $\nabla_\theta Q_{\theta}(A)$ can have very high dimensionality, we form an approximation and replace them with $\nabla_{\theta^{\text{last}}} Q_{\theta}(A)$, where $\theta^{\text{last}}$ denotes the parameters in the final layer of the $Q$-network (i.e. the parameters mapping the final hidden activations to the scalar value prediction). This change also has the convenience that $\nabla_{\theta^{\text{last}}} Q_{\theta}(A)$ is equal to the final hidden layer activations.



==> tables/different_ensembles.tex <==
\begin{table*}[h]
    \centering
    \begin{adjustbox}{center}
    {\small
    \begin{tabular}{|l||c||c||c|c|c|c||c||c|c|}
        \toprule
        Domain &  CQL & MSG & MIMO-0.5 & MIMO-1 & Multi-Head & Batch Ens & $N=1$ & Shared LCB & Shared Min\\
        \midrule
        halfcheetah-medium & 50.1 & 50.6 & 40.0& 44.4 & 49.8 & 40.2 & 48.6 & 47.9 & 36.0 \\
        hopper-medium & 90.2 & 88.2 & 60.2 & 65.1 & 94.8 & 41.6 & 50.2 & 30.0 & 43.6 \\
        walker2d-medium & 82.8 & 83.6 & 80.7 & 83.6 & 84.5 & 13.2 & 84.9 & 85.5 & 0.0 \\
        halfcheetah-mixed & 47.6 & 52.1 & 0.0 & 6.7 & 49.4 & 43.0 & 49.6 & 51.0 & 2.3 \\
        hopper-mixed & 61.1 & 82.1 & 22.7 & 32.5 & 45.5 & 35.0 & 30.5 & 32.5 & 6.7 \\
        walker2d-mixed & 20.5 & 24.0 & 14.5 & 16.8 & 15.9 & 12.0 & 11.5 & 26.3 & 0.0\\
        \midrule
        antmaze-large-diverse & 15.8 & 64.8 & 11.0 & 26.0 & 33.5 & 0.0 & 30.5 {\tiny (noisy)} & 0.0 & 0.0 \\
        antmaze-large-play & 14.9 & 68.8 & 7.5 & 20.5 & 27.5 & 0.0 & 11.0 {\tiny (noisy)} & 0.0 & 0.0\\
        % \midrule
        % Runtime (steps/sec) & & & & & & & & & \\
        \bottomrule
    \end{tabular}
    }
    \end{adjustbox}
    \caption{
    % \kamyar{For a lot of the ensembles alpha=1.0 was good which was on the boundary of the hyper= search, but no time to run more stuff. N=1 is pretty noisy, might need to run with more seeds. Also would be good to see how far we can push N=1 if we tuned the alpha.}
    Results for efficient ensembles and ensemble ablations.
    \kamyar{REMOVE THIS, REMOVE THIS, REMOVE THIS, REMOVE THIS}
    }
    \label{tab:ensembles_variations}
\end{table*}


==> tables/gym_d4rl.tex <==
\begin{table*}[h]
\setlength{\tabcolsep}{3pt}
\centering
\begin{adjustbox}{center}
{\small
\begin{tabular}{|l|c|cc|cc||ccc||c|}
\toprule
{Domain} &    BC & CQL & $\alpha$ & F-BRC (no bonus) & $\alpha$ & MSG ($N=64$) & $\beta$ & $\alpha$ & Data Top 25\\
\midrule
halfcheetah-medium        &  $36.1$ & $\bm{50.1 \pm 1.2}$ & 0 & $45.7 \pm 0.5$ & $0.01$ & $\bm{50.6 \pm 1.5}$ & 0 & 0 & $37.0 \pm 2.0$ \\
hopper-medium             &  $29.0$ & $90.2 \pm 10.5$ & $2.58$ &  $\bm{99.0 \pm 4.1}$ & $0.012$ & $88.2 \pm 11.6$ & -1 & 0.5 & $101.1 \pm 1.1$ \\ 
walker2d-medium           &   $6.6$ & $\bm{82.8 \pm 0.6}$ & $3.38$ &  $\bm{81.6 \pm 0.2}$ & 0.016 & $\bm{83.6 \pm 2.0}$ & -1 & 0.1 & $77.6 \pm 1.4$\\
\hline
halfcheetah-mixed         &  $38.4$ & $47.6 \pm 2.5$ & $0.67$ & $45.3 \pm 0.1$ & 0.01 & $\bm{52.1 \pm 1.7}$ & 0 & 0 & $38.1 \pm 4.1$ \\
hopper-mixed              &  $11.8$ &   $ 61.1 \pm 36.8 $ & $0.67$ &  $ 29.3 \pm 0.8$ & 0.019 & $\bm{82.1 \pm 24.2}$ & -2 & 0 & $101.8 \pm 1.5$\\
walker2d-mixed            &  $11.3$ &  $\bm{20.5 \pm 3.8}$ & $3.38$ & $\bm{28.4 \pm 5.7}$ & 0.038 &  $\bm{24.0 \pm 9.4}$ & -2 & 0.1 & $50.6 \pm 3.9$\\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\caption{\small
Results on Gym subset of the D4RL benchmark. For MSG we use an ensemble size of $N=64$. For fairness of comparison, F-BRC is ran without adding a survival reward bonus. For each method we also report the hyperparameter value used. Full experimental details are presented in Appendix \ref{app:gym_details}.
}
\label{tab:gym_results}
\end{table*}
%\footnotetext{The numbers for CQL here are taken directly from the results published in~\citet{kumar2020conservative}. However, we were not able to reproduce these ourselves with the author-provided open-source implementation, despite extensive correspondence with the first author of~\citet{kumar2020conservative}.}


==> what_is_generalization.tex <==
\section{What is generalization, and how do we measure it?}
    The notion of generalization in RL can be quite different than the one typically used in supervised learning. In supervised learning, generalization refers to the difference in loss between the training set, and the expected loss under iid samples from the task distribution. So there are two key questions we must first answer:
    \begin{enumerate}
        \item What do we mean by generalization in offline RL?
        \item How do we measure generalization in offline RL?
    \end{enumerate}
    
    \subsection{What?}
        \paragraph{Improving upon the trajectories in the dataset}
            
        
        \paragraph{Same Task, Different MDP from Same Family}
            Consider a family a MDPs, all of which share a common structure, and our aim is to solve the same task. Examples include, a robot opening doors in different building, a quadruped walking on different types of terrains, or a game playing agent solving different levels of a given game. In this scenario, an offline dataset may include interactions with a subset of MDPs in the family, and our hope is that offline agents can then "generalize" to unseen MDPs from the same task family.
        
        \paragraph{Solving a different task than what is being solved in the offline data}
            Sometimes, we may be interested in learning from past interactions in order to solve a new task. For example, a skateboarder can use their experience to figure out how to perform new tricks, knowledge gained from treating past illnesses can help us navigate new maladies, and .
    
    \subsection{How?}
        Given the types of generalization described above, an important question is "How do we quantitatively measure them?".
        
        \paragraph{Performance} The seemingly most straight-forward measure would be performance of trained agents in the desired transfer settings.
        
        \paragraph{Performance++} Many state-of-the-art offline RL methods follow an actor-critic framework. In these settings, it can be challenging to identify whether the performance in transfer settings is a results of good/bad transfer of the actor or the value functions. To better be able to understand the transfer ability of value functions, we can reformulate these algorithms in the setup used by EMaQ, where there is no explicit actor. Or, instead of EMaQ-style, at test-time we can sample multiple actions from the policy (and some from uniform) then pick the best under the Q-values.
        
        \paragraph{Measure the transfer of value estimate} Performance++ has the benefit of caring about the relative value estimates between different actions, instead of the actual value. To obtain a better picture, we could also measure the accuracy of the actual Q-values, by forming monte-carlo estimates of the policy in the transfer settings, and comparing to the predicted Q-values. For this, we do not need to 

    \subsection{Our Definition of Generalization in Offline RL}
    
    \subsection{How do we measure it?}
        \begin{itemize}
            \item V1: Same task at train and test time, different versions of the environment
            \item V2: Different task at test time from the tasks that generated the dataset
            \item V3: Actually comparing the Q-values, to monte carlo rollouts or something? Relative Q-values vs. actual Q-values?
        \end{itemize}
